Which $L_p$ norm is the fairest? Approximations for fair facility location across all "$p$"

Fair facility location problems try to balance access costs to open facilities borne by different groups of people by minimizing the $L_p$ norm of these group distances. However, there is no clear choice of "$p$" in the current literature. We present a novel approach to address the challenge of choosing the right notion of fairness. We introduce the concept of portfolios, a set of solutions that contains an approximately optimal solution for each objective in a given class of objectives, such as $L_p$ norms. This concept opens up new possibilities for getting around the "right" notion of fairness for many problems. For $r$ client groups, we demonstrate portfolios of size $\Theta(\log r)$ for the facility location and $k$-clustering problems, with an $O(1)$-approximate solution for each $L_p$ norm. Further, motivated by the Justice40 Initiative that provides rolling budget investments, we impose a refinement-like structure on the portfolio. We develop novel approximation algorithms for these structured portfolios and show experimental evidence of their performance in two US counties. We also present a planning tool that provides potential ways to expand access to US healthcare facilities, which might be of independent interest to policymakers.

==> images/line-example-a.tex <==
\tikzset{edge/.style = {->,> = latex'}}

\scriptsize

% \draw[gray, thick, -|] (-1,3) -- (0,3);
% \draw[gray, thick, -|] (0,3) -- (1,3);
% \draw[gray, thick, -|] (1,3) -- (2,3);
% \draw[gray, thick, -|] (2,3) -- (4,3);
% \draw[gray, thick] (4,3) -- (5,3);
\draw[black] (0,3) circle (0pt) node[anchor=north]{$0$};
\draw[black] (1,3) circle (0pt) node[anchor=north]{$1$};
\draw[black] (2,3) circle (0pt) node[anchor=north]{$2$};
\draw[black] (4,3) circle (0pt) node[anchor=north]{$4$};
        
\draw[] (0, -0.2) circle (0pt) node[anchor=north]{$f_0$};
\draw[] (1, -0.2) circle (0pt) node[anchor=north]{$f_1$};
\draw[] (2, -0.2) circle (0pt) node[anchor=north]{$f_2$};
\draw[] (4, -0.2) circle (0pt) node[anchor=north]{$f_4$};

\draw[gray, thick] (-1,0) -- (5,0);
\draw[gray, thick, dotted] (-2,0) -- (-1,0);
\draw[gray, thick, dotted] (5,0) -- (6,0);
\draw[black] (0,0) circle (0pt) node[]{$\times$};
\draw[black] (1,0) circle (0pt) node[]{$\times$};
\draw[black] (2,0) circle (0pt) node[]{$\times$};
\draw[black] (4,0) circle (0pt) node[]{$\times$};
\draw[blue, very thick, |-|] (-1,0) -- (0.25,0);
\draw[blue, very thick, |-|] (0.75,0) -- (1.25,0);
\draw[blue, very thick, |-|] (1.75,0) -- (2.5,0);
\draw[blue, very thick, |-|] (3.5,0) -- (5,0);

\draw[gray, thick] (-1,1) -- (5,1);
\draw[gray, thick, dotted] (-2,1) -- (-1,1);
\draw[gray, thick, dotted] (5,1) -- (6,1);
\draw[black] (0,1) circle (0pt) node[]{$\times$};
\draw[black] (4,1) circle (0pt) node[]{$\times$};
\draw[red, very thick, |-|] (-1,1) -- (1,1);
\draw[red, very thick, |-|] (3,1) -- (5,1);
% \draw[red, dotted, very thick] (1,1) -- (1.25,1);

\draw[gray, thick] (-1,2) -- (5,2);
\draw[gray, thick, dotted] (-2,2) -- (-1,2);
\draw[gray, thick, dotted] (5,2) -- (6,2);
\draw[black] (0,2) circle (0pt) node[]{$\times$};
\draw[ForestGreen, very thick, |-|] (-1,2) -- (5,2);

\draw[] (-3, 0) circle (0pt) node[]{$F_2$};
\draw[] (-3, 1) circle (0pt) node[]{$F_1$};
\draw[] (-3, 2) circle (0pt) node[]{$F_0$};

% \draw[edge, black] (0, 0.9) to (0, 0.1);
% \draw[edge, black] (0, 1.9) to (0, 1.1);
% \draw[edge, black] (0, 1.9)[bend left] to (2, 0.1);
% \draw[edge, black] (0, 1.9) to (4, 1.1);
% \draw[edge, black] (0, 0.9) to[bend left] (1, 0.1);
% \draw[edge, black] (4, 0.9) to (4, 0.1);

\draw[black] (2,-1.5) circle (0pt) node[]{(a)};


==> images/line-example-b.tex <==
\tikzset{edge/.style = {->,> = latex'}}

\scriptsize

\draw[black] (0,3) circle (0pt) node[anchor=north]{$0$};
\draw[black] (1,3) circle (0pt) node[anchor=north]{$1$};
\draw[black] (2,3) circle (0pt) node[anchor=north]{$2$};
\draw[black] (4,3) circle (0pt) node[anchor=north]{$4$};

\draw[] (0, -0.2) circle (0pt) node[anchor=north]{$f_0$};
\draw[] (1, -0.2) circle (0pt) node[anchor=north]{$f_1$};
\draw[] (2, -0.2) circle (0pt) node[anchor=north]{$f_2$};
\draw[] (4, -0.2) circle (0pt) node[anchor=north]{$f_4$};

\draw[gray, thick] (-1,0) -- (5,0);
\draw[gray, thick, dotted] (-2,0) -- (-1,0);
\draw[gray, thick, dotted] (5,0) -- (6,0);
\draw[black] (0,0) circle (0pt) node[]{$\times$};
\draw[black] (1,0) circle (0pt) node[]{$\times$};
\draw[black] (2,0) circle (0pt) node[]{$\times$};
\draw[black] (4,0) circle (0pt) node[]{$\times$};
\draw[blue, very thick, |-|] (-1,0) -- (0.25,0);
\draw[blue, very thick, |-|] (0.75,0) -- (1.25,0);
\draw[blue, very thick, |-|] (1.75,0) -- (2.5,0);
\draw[blue, very thick, |-|] (3.5,0) -- (5,0);

\draw[gray, thick] (-1,1) -- (5,1);
\draw[gray, thick, dotted] (-2,1) -- (-1,1);
\draw[gray, thick, dotted] (5,1) -- (6,1);
\draw[black] (0,1) circle (0pt) node[]{$\times$};
\draw[black] (4,1) circle (0pt) node[]{$\times$};
\draw[red, very thick, |-|] (-1,1) -- (1.25,1);
\draw[red, thick, dashed] (1,0.6) -- (1,1.4);
\draw[red, very thick, |-|] (3,1) -- (5,1);
% \draw[red, dotted, very thick] (1,1) -- (1.25,1);

\draw[gray, thick] (-1,2) -- (5,2);
\draw[gray, thick, dotted] (-2,2) -- (-1,2);
\draw[gray, thick, dotted] (5,2) -- (6,2);
\draw[black] (0,2) circle (0pt) node[]{$\times$};
\draw[ForestGreen, very thick, |-|] (-1,2) -- (5,2);

\draw[] (-3, 0) circle (0pt) node[]{$F_2$};
\draw[] (-3, 1) circle (0pt) node[]{$F_1$};
\draw[] (-3, 2) circle (0pt) node[]{$F_0$};

\draw[edge, black] (0, 0.9) to (0, 0.1);
\draw[edge, black] (0, 1.9) to (0, 1.1);
\draw[edge, black] (0, 1.9)[bend left] to (2, 0.1);
\draw[edge, black] (0, 1.9) to (4, 1.1);
\draw[edge, black] (0, 0.9) to[bend left] (1, 0.1);
\draw[edge, black] (4, 0.9) to (4, 0.1);
        
\draw[black] (2,-1.5) circle (0pt) node[]{(b)};


==> images/line-example-c.tex <==
\tikzset{edge/.style = {->,> = latex'}}

\scriptsize

\draw[black] (0,3) circle (0pt) node[anchor=north]{$0$};
\draw[black] (1,3) circle (0pt) node[anchor=north]{$1$};
\draw[black] (2,3) circle (0pt) node[anchor=north]{$2$};
\draw[black] (4,3) circle (0pt) node[anchor=north]{$4$};


\draw[] (0, -0.2) circle (0pt) node[anchor=north]{$f_0$};
\draw[] (1, -0.2) circle (0pt) node[anchor=north]{$f_1$};
\draw[] (2, -0.2) circle (0pt) node[anchor=north]{$f_2$};
\draw[] (4, -0.2) circle (0pt) node[anchor=north]{$f_4$};

\draw[gray, thick] (-1,0) -- (5,0);
\draw[gray, thick, dotted] (-2,0) -- (-1,0);
\draw[gray, thick, dotted] (5,0) -- (6,0);
\draw[black] (0,0) circle (0pt) node[]{$\times$};
\draw[black] (1,0) circle (0pt) node[]{$\times$};
\draw[black] (2,0) circle (0pt) node[]{$\times$};
\draw[black] (4,0) circle (0pt) node[]{$\times$};
\draw[blue, very thick, |-|] (-1,0) -- (0.25,0);
\draw[blue, very thick, |-|] (0.75,0) -- (1.25,0);
\draw[blue, very thick, |-|] (1.75,0) -- (2.5,0);
\draw[blue, very thick, |-|] (3.5,0) -- (5,0);

\draw[gray, thick] (-1,1) -- (5,1);
\draw[gray, thick, dotted] (-2,1) -- (-1,1);
\draw[gray, thick, dotted] (5,1) -- (6,1);
\draw[black] (0,1) circle (0pt) node[]{$\times$};
\draw[black] (4,1) circle (0pt) node[]{$\times$};
\draw[red, very thick, |-|] (-1,1) -- (2.5,1);
\draw[red, very thick, |-|] (3,1) -- (5,1);
% \draw[red, dotted, very thick] (1,1) -- (1.25,1);

\draw[gray, thick] (-1,2) -- (5,2);
\draw[gray, thick, dotted] (-2,2) -- (-1,2);
\draw[gray, thick, dotted] (5,2) -- (6,2);
\draw[black] (0,2) circle (0pt) node[]{$\times$};
\draw[ForestGreen, very thick, |-|] (-1,2) -- (5,2);

\draw[] (-3, 0) circle (0pt) node[]{$F_2$};
\draw[] (-3, 1) circle (0pt) node[]{$F_1$};
\draw[] (-3, 2) circle (0pt) node[]{$F_0$};

\draw[edge, black] (0, 0.9) to (0, 0.1);
\draw[edge, black] (0, 1.9) to (0, 1.1);
\draw[edge, gray, dashed] (0, 1.9)[bend left] to (2, 0.1);
\draw[edge, very thick, black] (0, 0.9)[bend left] to (2, 0.1);
\draw[edge, black] (0, 1.9) to (4, 1.1);
\draw[edge, black] (0, 0.9) to[bend left] (1, 0.1);
\draw[edge, black] (4, 0.9) to (4, 0.1);

\draw[black] (2,-1.5) circle (0pt) node[]{(c)};


==> images/line-example-d.tex <==
\tikzset{edge/.style = {->,> = latex'}}

\scriptsize

\draw[black] (0,3) circle (0pt) node[anchor=north]{$0$};
\draw[black] (1,3) circle (0pt) node[anchor=north]{$1$};
\draw[black] (2,3) circle (0pt) node[anchor=north]{$2$};
\draw[black] (4,3) circle (0pt) node[anchor=north]{$4$};


\draw[] (0, -0.2) circle (0pt) node[anchor=north]{$f_0$};
\draw[] (1, -0.2) circle (0pt) node[anchor=north]{$f_1$};
\draw[] (2, -0.2) circle (0pt) node[anchor=north]{$f_2$};
\draw[] (4, -0.2) circle (0pt) node[anchor=north]{$f_4$};

\draw[gray, thick] (-1,0) -- (5,0);
\draw[gray, thick, dotted] (-2,0) -- (-1,0);
\draw[gray, thick, dotted] (5,0) -- (6,0);
\draw[black] (0,0) circle (0pt) node[]{$\times$};
\draw[black] (1,0) circle (0pt) node[]{$\times$};
\draw[black] (2,0) circle (0pt) node[]{$\times$};
\draw[black] (4,0) circle (0pt) node[]{$\times$};
\draw[blue, very thick, |-] (-1,0) -- (0.5,0);
\draw[blue, very thick, |-] (0.5,0) -- (1.5,0);
\draw[blue, very thick, |-] (1.5,0) -- (2.7,0);
\draw[blue, very thick, |-|] (2.7,0) -- (5,0);

\draw[gray, thick] (-1,1) -- (5,1);
\draw[gray, thick, dotted] (-2,1) -- (-1,1);
\draw[gray, thick, dotted] (5,1) -- (6,1);
\draw[black] (0,1) circle (0pt) node[]{$\times$};
\draw[black] (4,1) circle (0pt) node[]{$\times$};
\draw[red, very thick, |-] (-1,1) -- (2.7,1);
\draw[red, very thick, |-|] (2.7,1) -- (5,1);
% \draw[red, dotted, very thick] (1,1) -- (1.25,1);

\draw[gray, thick] (-1,2) -- (5,2);
\draw[gray, thick, dotted] (-2,2) -- (-1,2);
\draw[gray, thick, dotted] (5,2) -- (6,2);
\draw[black] (0,2) circle (0pt) node[]{$\times$};
\draw[ForestGreen, very thick, |-|] (-1,2) -- (5,2);

\draw[] (-3, 0) circle (0pt) node[]{$F_2$};
\draw[] (-3, 1) circle (0pt) node[]{$F_1$};
\draw[] (-3, 2) circle (0pt) node[]{$F_0$};

\draw[edge, black] (0, 0.9) to (0, 0.1);
\draw[edge, black] (0, 1.9) to (0, 1.1);
% \draw[edge, gray!50] (0, 1.9)[bend left] to (2, 0.1);
\draw[edge, black] (0, 0.9)[bend left] to (2, 0.1);
\draw[edge, black] (0, 1.9) to (4, 1.1);
\draw[edge, black] (0, 0.9) to[bend left] (1, 0.1);
\draw[edge, black] (4, 0.9) to (4, 0.1);

\draw[black] (2,-1.5) circle (0pt) node[]{(d)};

